VecFusion: Vector Font Generation with Diffusion

We present VecFusion, a new neural architecture that can generate vector fonts with varying topological structures and precise control point positions. Our approach is a cascaded diffusion model which consists of a raster diffusion model followed by a vector diffusion model. The raster model generates low-resolution, rasterized fonts with auxiliary control point information, capturing the global style and shape of the font, while the vector model synthesizes vector fonts conditioned on the low-resolution raster fonts from the first stage. To synthesize long and complex curves, our vector diffusion model uses a transformer architecture and a novel vector representation that enables the modeling of diverse vector geometry and the precise prediction of control points. Our experiments show that, in contrast to previous generative models for vector graphics, our new cascaded vector diffusion model generates higher quality vector fonts, with complex structures and diverse styles.

==> figures/CVPR/5_results_fewshot.tex <==
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{2}

    % \setlength{\arrayrulewidth}{0.3pt}
    
    \begin{tabular}{llll | c c c}
        \multicolumn{4}{c}{Input reference} &  (a) & (b) & (c)\\
        % \hline
        % &  & &  \\
\includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4483_ref0.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4483_ref1.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4483_ref2.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4483_ref3.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4483_gt.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4483_ours.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4483_dvfv2.pdf}   \\
\includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/2546_ref0.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/2546_ref1.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/2546_ref2.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/2546_ref3.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/2546_gt.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/2546_ours.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/2546_dvfv2.pdf}  
 \\
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/70_ref0.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/70_ref1.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/70_ref2.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/70_ref3.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/70_gt.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/70_ours.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/70_dvfv2.pdf}   \\

 \includegraphics[height=0.05\textwidth,width=0.05\textwidth]{images/few_shot_gen/CVPR/pdfs/4343_ref0.pdf} 
&
 \includegraphics[height=0.05\textwidth,width=0.05\textwidth]{images/few_shot_gen/CVPR/pdfs/4343_ref1.pdf} 
&
 \includegraphics[height=0.05\textwidth,width=0.05\textwidth]{images/few_shot_gen/CVPR/pdfs/4343_ref2.pdf} 
&
 \includegraphics[height=0.05\textwidth,width=0.05\textwidth]{images/few_shot_gen/CVPR/pdfs/4343_ref3.pdf} 
&
 \includegraphics[height=0.05\textwidth,width=0.05\textwidth]{images/few_shot_gen/CVPR/pdfs/4343_gt.pdf} 
&
 \includegraphics[height=0.05\textwidth,width=0.05\textwidth]{images/few_shot_gen/CVPR/pdfs/4343_ours.pdf} 
&
 \includegraphics[height=0.05\textwidth,width=0.05\textwidth]{images/few_shot_gen/CVPR/pdfs/4343_dvfv2.pdf}   \\
\includegraphics[height=0.06\textwidth,width=0.06\textwidth]{images/few_shot_gen/CVPR/pdfs/2215_ref0.pdf} 
&
 \includegraphics[height=0.05\textwidth,width=0.05\textwidth]{images/few_shot_gen/CVPR/pdfs/2215_ref1.pdf} 
&
 \includegraphics[height=0.06\textwidth,width=0.06\textwidth]{images/few_shot_gen/CVPR/pdfs/2215_ref2.pdf} 
&
 \includegraphics[height=0.06\textwidth,width=0.06\textwidth]{images/few_shot_gen/CVPR/pdfs/2215_ref3.pdf} 
&
 \includegraphics[height=0.06\textwidth,width=0.06\textwidth]{images/few_shot_gen/CVPR/pdfs/2215_gt.pdf} 
&
 \includegraphics[height=0.06\textwidth,width=0.06\textwidth]{images/few_shot_gen/CVPR/pdfs/2215_ours.pdf} 
&
 \includegraphics[height=0.06\textwidth,width=0.06\textwidth]{images/few_shot_gen/CVPR/pdfs/2215_dvfv2.pdf}   \\
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/8_ref0.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/8_ref1.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/8_ref2.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/8_ref3.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/8_gt.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/8_ours.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/8_dvfv2.pdf}   \\
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4842_ref0.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4842_ref1.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4842_ref2.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4842_ref3.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4842_gt.pdf} 
&
\includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4842_ours.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4842_dvfv2.pdf}   \\
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4000_ref0.pdf} 
&
 \includegraphics[height=0.05\textwidth,width=0.05\textwidth]{images/few_shot_gen/CVPR/pdfs/4000_ref1.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4000_ref2.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4000_ref3.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4000_gt.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4000_ours.pdf} 
&
 \includegraphics[height=0.055\textwidth,width=0.055\textwidth]{images/few_shot_gen/CVPR/pdfs/4000_dvfv2.pdf}   \\
    \end{tabular}
    \vspace{-1mm}
    \caption{Few-shot style transfer results. On the left, we show the reference glyphs belonging to a novel font style. On the right, we show (a) the artist-made (``ground-truth'') glyphs, (b) our generated ones, and (c) the ones produced by DeepVecFont-v2 \cite{wang2023deepvecfont}. \label{fig:font_style_transfer}}
    \vspace{-1em}
\end{figure}


==> tables/SA/1_vectorization.tex <==
\begin{table}[t!]
    \centering
    \small
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lcccc}
         \toprule
         \textbf{Method} & \textbf{L2 $\downarrow$} & \textbf{Curve-to-curve distance $\downarrow$}& \textbf{SSIM $\uparrow$}
         \\
         \midrule
        Ours 
        &  &   &   & \\
        DeepSVG \cite{carlier2020deepsvg}
        &  &   &   & \\
        ChiroDiff \cite{das2023chirodiff}
        &  &   &   & \\
        Im2Vec \cite{reddy2021im2vec}
        &  &   &   & \\
        Least-squares fitting
        &  &   &   & \\
         \bottomrule
    \end{tabular}
    \caption{Vectorization results}
    \label{tab:vectorization}
\end{table}

==> tables/SA/2_fewshot_generation.tex <==
\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l ccccc}
         \toprule
         \textbf{Method} & $L_1$ $\downarrow$ & CD $\downarrow$ & \#cp diff $\downarrow$ & \#vp diff $\downarrow$
         \\
         \midrule
        Ours 
        & \textbf{0.069} & \textbf{0.46}  & \textbf{15.05} & \textbf{0.033} \\
        DeepVecFont-v2 \cite{wang2023deepvecfont}
        & 0.098 & 1.05  & 34.84 & 0.052 \\
         \bottomrule
    \end{tabular}
    \vspace{-3mm}
    \caption{\rev{Few-shot font style transfer evaluation.}}
    % CD is scaled by $10^2$.
    \label{tab:font_style_transfer}
    \vspace{-5mm}
\end{table}


==> tables/SA/3_unconditional_generation.tex <==
\begin{table}[t!]
    \centering
    \small
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lcccc}
         \toprule
         \textbf{Method} & \textbf{FID $\downarrow$}
         \\
         \midrule
        Ours 
        &  &   &   & \\
        DeepSVG \cite{carlier2020deepsvg}
        &  &   &   & \\
        ChiroDiff \cite{das2023chirodiff}
        &  &   &   & \\
        Im2Vec \cite{reddy2021im2vec}
        &  &   &   & \\
        DeepVecFont \cite{wang2021deepvecfont}
        &  &   &   & \\
         \bottomrule
    \end{tabular}
    \caption{Unconditional generation results}
    \label{tab:uncond_generation}
\end{table}
